Zip-NeRF: Anti-Aliased Grid-Based Neural Radiance Fields

Neural Radiance Field training can be accelerated through the use of grid-based representations in NeRF's learned mapping from spatial coordinates to colors and volumetric density. However, these grid-based approaches lack an explicit understanding of scale and therefore often introduce aliasing, usually in the form of jaggies or missing scene content. Anti-aliasing has previously been addressed by mip-NeRF 360, which reasons about sub-volumes along a cone rather than points along a ray, but this approach is not natively compatible with current grid-based techniques. We show how ideas from rendering and signal processing can be used to construct a technique that combines mip-NeRF 360 and grid-based models such as Instant NGP to yield error rates that are 8% - 77% lower than either prior technique, and that trains 24x faster than mip-NeRF 360.

==> tables/ablation.tex <==
& mip-NeRF 360 + iNGP             &                   26.53 &                   0.774 &                   0.252 &                   27.99 &                   0.856 &                   0.140 &                   27.72 &                   0.867 &                   0.115 &                   25.61 &                   0.804 &                   0.159 & 0.32 \\
\hline
& Our Model                       & \cellcolor{yellow}28.20 & \cellcolor{yellow}0.822 &                   0.200 &    \cellcolor{red}29.94 &    \cellcolor{red}0.892 &    \cellcolor{red}0.099 & \cellcolor{orange}31.48 &    \cellcolor{red}0.933 &    \cellcolor{red}0.056 &    \cellcolor{red}32.40 &    \cellcolor{red}0.954 &    \cellcolor{red}0.038 & 0.97 \\
\hline
A) & No Weight Decay              &                   26.64 &                   0.805 &                   0.214 &                   28.19 &                   0.871 &                   0.120 &                   29.53 &                   0.908 &                   0.081 &                   30.44 &                   0.927 &                   0.064 & 0.96 \\
B) & Un-Normalized Weight Decay   &                   27.91 &                   0.820 & \cellcolor{yellow}0.199 &                   29.55 &                   0.888 &                   0.102 &                   30.98 & \cellcolor{yellow}0.929 &                   0.059 &                   31.93 &                   0.950 &                   0.041 & 0.97 \\
C) & Small MLP                    &                   27.38 &                   0.811 &                   0.210 &                   28.95 &                   0.882 &                   0.109 &                   30.26 &                   0.923 &                   0.065 &                   31.01 &                   0.944 &                   0.048 & 0.68 \\
D) & No Multisampling             &                   28.13 &                   0.816 &                   0.210 &                   29.83 &                   0.886 &                   0.106 &                   31.29 &                   0.927 &                   0.061 & \cellcolor{yellow}32.06 &                   0.947 &                   0.043 & 0.56 \\
E) & No Downweighting             & \cellcolor{yellow}28.20 &                   0.817 &                   0.208 & \cellcolor{yellow}29.91 &                   0.888 &                   0.103 &                   31.05 &                   0.926 &                   0.062 &                   31.17 &                   0.941 &                   0.051 & 0.93 \\
F) & Naive Sampling               &                   27.90 &                   0.796 &                   0.234 &                   29.67 &                   0.880 &                   0.115 &                   29.20 &                   0.887 &                   0.095 &                   26.51 &                   0.820 &                   0.144 & 0.56 \\
G) & Naive Sampling (4x samples)  &                   27.65 &                   0.803 &                   0.225 &                   29.28 &                   0.884 &                   0.109 &                   28.68 &                   0.884 &                   0.095 &                   26.11 &                   0.814 &                   0.148 & 1.71 \\
H) & No Multiscale Training       &    \cellcolor{red}28.25 &    \cellcolor{red}0.826 &    \cellcolor{red}0.192 &                   24.91 &                   0.811 &                   0.156 &                   20.84 &                   0.702 &                   0.219 &                   18.54 &                   0.627 &                   0.267 & 0.96 \\
I) & No New Interlevel Loss       &                   28.04 & \cellcolor{orange}0.823 & \cellcolor{orange}0.198 &                   29.73 &    \cellcolor{red}0.892 &    \cellcolor{red}0.099 &                   31.18 & \cellcolor{orange}0.932 & \cellcolor{orange}0.057 &                   32.01 & \cellcolor{yellow}0.952 & \cellcolor{yellow}0.040 & 0.94 \\
J) & Random Multisampling (7, 7)  &                   28.09 &                   0.816 &                   0.206 &                   29.74 &                   0.886 &                   0.105 &                   31.18 &                   0.928 &                   0.061 & \cellcolor{yellow}32.06 &                   0.950 &                   0.042 & 1.04 \\
K) & Random Multisampling (7, 49) & \cellcolor{orange}28.21 &                   0.820 &                   0.204 & \cellcolor{orange}29.93 & \cellcolor{yellow}0.890 &                   0.102 & \cellcolor{yellow}31.45 & \cellcolor{orange}0.932 & \cellcolor{yellow}0.058 & \cellcolor{orange}32.31 & \cellcolor{orange}0.953 & \cellcolor{yellow}0.040 & 1.04 \\
L) & Julier Multisampling         & \cellcolor{orange}28.21 &                   0.821 &                   0.200 &    \cellcolor{red}29.94 & \cellcolor{orange}0.891 & \cellcolor{orange}0.100 &    \cellcolor{red}31.50 & \cellcolor{orange}0.932 &    \cellcolor{red}0.056 &    \cellcolor{red}32.40 & \cellcolor{orange}0.953 & \cellcolor{orange}0.039 & 1.12 \\
M) & Julier/Spiral Multisampling  &                   28.04 &                   0.819 &                   0.200 &                   29.69 &                   0.887 & \cellcolor{yellow}0.101 &                   31.07 &                   0.927 &                   0.060 &                   31.68 &                   0.945 &                   0.046 & 1.12
